Model-Free Characterizations of the Hamilton-Jacobi-Bellman Equation and Convex Q-Learning in Continuous Time

Convex Q-learning is a recent approach to reinforcement learning, motivated by the possibility of a firmer theory for convergence, and the possibility of making use of greater a priori knowledge regarding policy or value function structure. This paper explores algorithm design in the continuous time domain, with finite-horizon optimal control objective. The main contributions are (i) Algorithm design is based on a new Q-ODE, which defines the model-free characterization of the Hamilton-Jacobi-Bellman equation. (ii) The Q-ODE motivates a new formulation of Convex Q-learning that avoids the approximations appearing in prior work. The Bellman error used in the algorithm is defined by filtered measurements, which is beneficial in the presence of measurement noise. (iii) A characterization of boundedness of the constraint region is obtained through a non-trivial extension of recent results from the discrete time setting. (iv) The theory is illustrated in application to resource allocation for distributed energy resources, for which the theory is ideally suited.

==> bookmacrosRL_IEEE.tex <==
     \makeatletter
\newcommand\gobblepars{%
    \@ifnextchar\par%
        {\expandafter\gobblepars\@gobble}%
        {}}
\makeatother

\def\head#1{\par\noindent\textbf{#1} \ \gobblepars}

\def\Shead#1{\smallbreak\noindent\textbf{\textit{#1}} \ \gobblepars}



%%%%%%%%%%%%%%%%%%%%%%
\def\mindex#1{\index{#1}}

% symbol index - definition to be created
\def\sindex#1{\index{{ }#1}}

%\typeout{REMOVE SINDEX AND MINDEX AT END}
%\typeout{CHECK NOTES IN SPRINGER3}

\def\breakMed{\\[.2cm]}
\def\breakBig{\\[.35cm]}

 \def\oc{\star}   % for optimal control
\def\ocp{*}   % for optimal parameter or function approximation
  
 \def\baru{\bar{u}}
 
 


%\newenvironment{ex}{\begin{example}}{\qed\end{example}}


%%%  QSA notation  

\def\tilnabla{{\widetilde{\nabla}\!}}
%
%\newcommand{\varqsa}{\theta}
%\def\varqsaPR{\varqsa^{\text{PR}}}

%%%%%%%%%%%  QSA  %%%%%%%%%%%  
 

\newcommand{\qsaprobe}{{\scalebox{1.1}{$\upxi$}}}  %\upzeta \textphi
\newcommand{\bfqsaprobe}{{\scalebox{1.1}{$\bm{\upxi}$}}}  

\newcommand{\qsaprobeTwo}{\qsaprobe^\bullet}  % 

\def\SAtime{\uptau}

%%%%%%%%%%%%

\def\lipConstant{\ell}
\def\Obj{L}
 
\def\Evo{\mathcal{X}} 


%%%  RL notation
\def\tERM{{\text{\tiny ERM}}}


\def\density{p}

\def\RateFn{\bar{I}}

\def\diffDPT{D}

\def\Amap{a}


\def\BE{{\cal B}}
\def\maxBE{\overline{\cal B}}

\def\Tdiff{\mathcal{D}}
\def\barTdiff{\bar{\mathcal{D}}}



\def\preODEstate{\Upxi} %\Upxi  \Upupsilon
\def\bfpreODEstate{\bm{\Upxi}}
\def\barpreODEstate{\bar{\Upxi}}
\def\tilpreODEstate{\tilde{\Upxi}}
\def\hatpreODEstate{\widehat{\Upxi}}
\def\bfhatpreODEstate{\hat{\bfpreODEstate}}


\def\ODEstate{\Uptheta} %\xi
\def\bfODEstate{\bm{\Uptheta}}
\def\barODEstate{\bar{\Uptheta}}
\def\tilODEstate{\tilde{\Uptheta}}
\def\hatODEstate{\widehat{\Uptheta}}
\def\bfhatODEstate{\widehat{\bfODEstate}}


\def\odestate{\upvartheta}
\def\bfodestate{\bm{\upvartheta}} 


\def\Nsam{N}

\def\belief{\text{\large$\beta$}}

\def\fee{\upphi}


\def\feex{{\breve{\fee}}} 

 \def\feeF{\phi^{\hbox{\tiny \rm F}}}
 \def\feeD{\phi^{\hbox{\tiny \rm D}}}
 
\def\Hor{\mathcal{T}} %H}
\def\hor{\uptau}   %\iota}



\def\pie{\varpi}



\def\elig{\zeta}
\def\bfelig{\bfmath{\zeta}}


\def\uc{\underline{c}}

\def\uh{\underline{h}}
\def\uq{\underline{q}}

\def\uH{\underline{H}}
\def\uQ{\underline{Q}}
\def\utheta{\underline{\theta}}  
  
\def\discRate{\Gamma}
\def\disc{\gamma}

 
\def\stepf{\beta}

%%%%%%%%%%%%%%%%%%%
 %%%%%% Special symbols
 
 
\def\mm{\phantom{-}}
  
  \def\mm{\phantom{-}}
  
 
 
 
\def\tinyrm#1{{\mathchoice{\mbox{\rm #1}}%
{\mbox{\rm #1}}%
{\mbox{\tiny \rm #1}}%
{\mbox{\tiny \rm #1}}}}

\def\mrmS{\tinyrm{S}}

\def\MW{{\mathchoice{\mbox{\rm MW}}%
{\mbox{\rm MW}}%
{\mbox{\tiny \rm MW}}%
{\mbox{\tiny \rm MW}}}}


 
 
 
 
\newcommand{\bbblot}{\raise1pt\hbox{\vrule height .4ex width .4ex depth .05ex}}
%\def\cGam{c^{\hbox{\tiny $\Gamma$}}} 
%\def\cGam{c^{\hbox{\tiny [\,]}}}
\def\cGam{c^{\hbox{\bbblot}}}

\def\tinyW{\hbox{\tiny W}}

\def\lbfs{{\mathchoice{\mbox{\rm LBFS}}%
{\mbox{\rm LBFS}}%
{\mbox{\tiny \rm LBFS}}%
{\mbox{\tiny \rm LBFS}}}}


 
 \def\PS{\hbox{\sf PS}}
 \def\PSm{\hbox{\sf PS}^{\hbox{\tiny{\sf M}}}}                                   % Policy space
\def\PSs{\hbox{\sf PS}^{\hbox{\tiny{\sf S}}}}                                      % Policy space
\def\PSr{\hbox{\sf PS}^{\hbox{\tiny{\sf RS}}}}                                   % Policy space
 

 
\def\bfPSm{\hbox{\bf PS}^{\hbox{\tiny{\sf M}}}}                                   % Policy space
\def\bfPSs{\hbox{\bf PS}^{\hbox{\tiny{\sf S}}}}                                   % Policy space
  
 \def\bfPS{\hbox{\textbf{\sf PS}}}
 
  

\def\mttf{{\hbox{\tiny MTTF}}}
\def\mttr{{\hbox{\tiny MTTR}}}

\def\fluid{{\hbox{\tiny fluid}}}
\def\gto{{\hbox{\tiny GTO}}}
\def\gtodr{{\hbox{\tiny GTO-DR}}}
\def\sto{{\hbox{\tiny STO}}}
 

\def\cDR{c_{\hbox{\tiny DR}}}
 
 \def\Didle{{\mathchoice{\mbox{\Large$\iota$}}%
 {\mbox{\Large$\iota$}}%
 {\mbox{\small\boldmath$\iota$}}%
 {\mbox{\small$\iota$}}}}
 
 \def\bfDidle{{\mathchoice{\mbox{\Large\boldmath$\iota$}}%
 {\mbox{\Large\boldmath$\iota$}}%
 {\mbox{\small\boldmath$\iota$}}%
 {\mbox{\small\boldmath$\iota$}}}}
 
  \def\haDidle{{\mathchoice{\widehat{\mbox{\Large$\iota$}}}%
 {\widehat{\mbox{\Large$\iota$}}}%
 {\widehat{\mbox{\small\boldmath$\iota$}}}%
 {\widehat{\mbox{\small$\iota$}}}}}
  
 \def\bfhaDidle{\widehat{\bfDidle}}  
 
 \def\bfidle{\mbox{\small\boldmath$I$}}
 \def\idle{\mbox{\small$I$}}
 
  \def\idle{{\mathchoice{\mbox{\small$I$}}%
 {\mbox{\small $I$}}%
 {\mbox{\small$I$}}%
 {\mbox{\tiny$I$}}}}
 
  \def\bfidle{{\mathchoice{\mbox{\small\boldmath$I$}}%
 {\mbox{\small \boldmath$I$}}%
 {\mbox{\small\boldmath$I$}}%
 {\mbox{\tiny\boldmath$I$}}}}
 

\def\haiota{\hat{\iota}}


\def\slPi{{\mit\Pi}}

\def\contains{\supset}
 
\def\LV{L_\infty^V} 
\def\Lf{L_\infty^f}
\def\LF{L_\infty^F}
\def\LW{L_\infty^{W}} 

 
  

 

%%%%%%%%%%%%%%%%%%FOR DEFINITIONS
       

\long\def\defbox#1{\framebox[.9\hsize][c]{\parbox{.85\hsize}{%
\parindent=0pt
\baselineskip=12pt plus .1pt      % STYLE 
\parskip=6pt plus 1.5pt minus 1pt % CHANGES
 #1}}}


%% Much improved beginbox:

\long\def\beginbox#1\endbox{\subsection*{}%
\hbox{\hspace{.05\hsize}\defbox{\medskip#1\bigskip}}%
\subsection*{}}

\def\endbox{}

%%%%%%%%%%%%%%%%%%% Notes
 
 \def\archival#1{} %Notes I'd like to save
 


\def\STOP{\typeout{RESUME EDITING HERE}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATH OPERATORS



\def\llangle{\langle\!\langle}
\def\rrangle{\rangle\!\rangle}

\def\llbracket{[\![}
\def\rrbracket{]\!]}




%%\genfrac{}{}{}{1}{1}{2} The \genfrac command is valid only in math mode.  
%It takes six arguments, say L, R, w, s, N, D. The translation is a fraction N over D,
% with left and right delimiters L and R. The parameter w specifies  the width of the
%  fraction rule. It can be omitted. The parameter s specifies the style, it is a number 
%  between 0 and 3, interpreted as  \displaystyle, \textstyle, scriptstyle  \scriptscriptstyle. 
%  It can be empty.  




\def\choose#1#2{{\mathchoice{\genfrac{(}{)}{0pt}{0}{#1}{#2}}%
{\genfrac{(}{)}{0pt}{1}{#1}{#2}}%
{\genfrac{(}{)}{0pt}{3}{#1}{#2}}%
{\genfrac{(}{)}{0pt}{3}{#1}{#2}}}}

\def\atopss#1#2{\genfrac{}{}{0cm}{2}{#1}{#2}} 

\def\atop#1#2{\genfrac{}{}{0pt}{}{#1}{#2}}
 
\def\FRAC#1#2#3{\genfrac{}{}{}{#1}{#2}{#3}}

 

\def\fraction#1#2{{\mathchoice{\FRAC{0}{#1}{#2}}%
{\FRAC{1}{#1}{#2}}%
{\FRAC{3}{#1}{#2}}%
{\FRAC{3}{#1}{#2}}}}


\def\ddt{{\mathchoice{\FRAC{1}{d}{dt}}%
{\FRAC{1}{d}{dt}}%
{\FRAC{3}{d}{dt}}%
{\FRAC{3}{d}{dt}}}}



\def\ddu{{\mathchoice{\FRAC{1}{d}{du}}%
{\FRAC{1}{d}{du}}%
{\FRAC{3}{d}{du}}%
{\FRAC{3}{d}{du}}}}

 

 
 


\def\ddx{{\mathchoice{\FRAC{1}{d}{dx}}%
{\FRAC{1}{d}{dx}}%
{\FRAC{3}{d}{dx}}%
{\FRAC{3}{d}{dx}}}}


\def\ddy{{\mathchoice{\FRAC{1}{d}{dy}}%
{\FRAC{1}{d}{dy}}%
{\FRAC{3}{d}{dy}}%
{\FRAC{3}{d}{dy}}}}


\def\ddw{{\mathchoice{\FRAC{1}{d}{dw}}%
{\FRAC{1}{d}{dw}}%
{\FRAC{3}{d}{dw}}%
{\FRAC{3}{d}{dw}}}}

\def\ddtheta{{\mathchoice{\FRAC{1}{d}{d\theta}}%
{\FRAC{1}{d}{d\theta}}%
{\FRAC{3}{d}{d\theta}}%
{\FRAC{3}{d}{d\theta}}}}

\def\ddr{{\mathchoice{\FRAC{1}{d}{dr}}%
{\FRAC{1}{d}{dr}}%
{\FRAC{3}{d}{dr}}%
{\FRAC{3}{d}{dr}}}}

\def\ddtp{{\mathchoice{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}}}

\def\ddyp{{\mathchoice{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dy}}%
{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dy}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dy}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dy}}}}


\def\half{{\mathchoice{\FRAC{1}{1}{2}}%
{\FRAC{1}{1}{2}}%
{\FRAC{3}{1}{2}}%
{\FRAC{3}{1}{2}}}}

\def\third{{\mathchoice{\FRAC{1}{1}{3}}%
{\FRAC{1}{1}{3}}%
{\FRAC{3}{1}{3}}%
{\FRAC{3}{1}{3}}}}

\def\fourth{{\mathchoice{\FRAC{1}{1}{4}}%
{\FRAC{1}{1}{4}}%
{\FRAC{3}{1}{4}}%
{\FRAC{3}{1}{4}}}}

\def\fifth{{\mathchoice{\FRAC{1}{1}{5}}%
{\FRAC{1}{1}{5}}%
{\FRAC{3}{1}{5}}%
{\FRAC{3}{1}{5}}}}

\def\twofifth{{\mathchoice{\FRAC{1}{2}{5}}%
{\FRAC{1}{2}{5}}%
{\FRAC{3}{2}{5}}%
{\FRAC{3}{2}{5}}}}

\def\threefifth{{\mathchoice{\FRAC{1}{3}{5}}%
{\FRAC{1}{3}{5}}%
{\FRAC{3}{3}{5}}%
{\FRAC{3}{3}{5}}}}

\def\threehalf{{\mathchoice{\FRAC{1}{3}{2}}%
{\FRAC{1}{3}{2}}%
{\FRAC{3}{3}{2}}%
{\FRAC{3}{3}{2}}}}

\def\threefourth{{\mathchoice{\FRAC{1}{3}{4}}%
{\FRAC{1}{3}{4}}%
{\FRAC{3}{3}{4}}%
{\FRAC{3}{3}{4}}}}
 

\def\sixth{{\mathchoice{\FRAC{1}{1}{6}}%
{\FRAC{1}{1}{6}}%
{\FRAC{3}{1}{6}}%
{\FRAC{3}{1}{6}}}}

\def\eighth{{\mathchoice{\FRAC{1}{1}{8}}%
{\FRAC{1}{1}{8}}%
{\FRAC{3}{1}{8}}%
{\FRAC{3}{1}{8}}}}


 

\def\Chi{{\mathchoice{\mbox{\Large $\chi$}}%
{\mbox{\Large $\chi$}}%
{\mbox{\normalsize   $\chi$}}%
{\mbox{\small   $\chi$}}}}



\def\gGamma{{\mathchoice{\mbox{\small $\Gamma$}}%
{\mbox{\small $\Gamma$}}%
{\mbox{\tiny   $\Gamma$}}%
{\mbox{\tiny   $\Gamma$}}}}

%  buildrel uses \over

\def\wkarrow{\buildrel{\rm w}\over\longrightarrow}
\def\vgarrow{\buildrel{\rm v}\over\longrightarrow}

\def\tvlimit#1{\buildrel{\scriptscriptstyle #1}\over\Longrightarrow}
\def\darrow{\buildrel{\rm d}\over\longrightarrow}

%\def\darrow{\buildrel{\rm d}\over\longrightarrow}

\def\eqdist{\buildrel{\rm dist}\over =}



\def\goes#1{\buildrel{#1}\over\longrightarrow}
\def\wiggles#1{\buildrel{#1}\over\leadsto}


\def\tr{{\rm tr\, }}

\def\rank{{\rm rank\,}}
\def\deg{\hbox{\rm deg\thinspace}}
\def\sign{{\rm sign}}
\def\supp{{\rm supp\,}}



\newsavebox{\junk}
\savebox{\junk}[1.6mm]{\hbox{$|\!|\!|$}}
\def\lll{{\usebox{\junk}}} 


\def\det{{\mathop{\rm det}}}
\def\limsup{\mathop{\rm lim{\,}sup}}
\def\liminf{\mathop{\rm lim{\,}inf}}
\def\argmin{\mathop{\rm arg{\,}min}}
\def\argmax{\mathop{\rm arg{\,}max}}
  
  
\def\esssup{\mathop{\rm ess{\,}sup}}
\def\essinf{\mathop{\rm ess{\,}inf}}

\def\bfmin{\mathop{\hbox{\bf min\,}}}
\def\bfmax{\mathop{\hbox{\bf max\, }}}
\def\bfargmin{\mathop{\hbox{\bf arg{\,}min\, }}}
\def\bfargmax{\mathop{\hbox{\bf arg{\,}max\, }}}

\def\bfst{\hbox{\bf s.{\,}t.\ }}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Control



\def\Dds{\text{\rm F}}
\def\Ddo{\text{\rm G}}

% Fluid model

\def\barDds{\overline{\text{\rm F}}}
\def\barDcs{\bar{\text{\rm f}}}

% Just for IMP
\def\Ddsm{\text{\rm F}_{\text{m}}}
\def\Ddom{\text{\rm G}_{\text{m}}}
 


\def\Dcs{\text{\rm f}}
\def\Dco{\text{\rm g}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPACES
 
 



\def\state{{\sf X}}

\def\bstate{\mathcal{X}}  %belief state

\def\ustate{{\sf U}} 
\def\ystate{{\sf Y}} 
\def\zstate{{\sf Z}} 
 

\def\dstateM{{\sf X_\diamond^{\hbox{\tiny \rm M}}}}
\def\piM{\pi^{\hbox{\tiny \rm M}}}
\def\phiM{\phi^{\hbox{\tiny \rm M}}}


\def\tilstate{{\sf \widetilde{X}}}

\def\tinyMathX{{\hbox{\it\tiny X}}}

\def\bx{{{\cal B}(\state)}}

\def\ystate{{\sf Y}}
\def\dystate{{\sf Y_\diamond}}

\def\sS{{\sf S}}

%\def\smallsfX{{\hbox{\scriptsize\sf X}}}
%\def\sfX{{\hbox{\sf X}}}
%\def\state{{\mathchoice\sfX\sfX\smallsfX\smallsfX}}


%\def\smallsfY{{\hbox{\scriptsize\sf Y}}}
%\def\sfY{{\hbox{\sf Y}}}
%\def\ystate{{\mathchoice\sfY\sfY\smallsfY\smallsfY}}

\def\by{\clB(\ystate)}

\def\tinyplus{\vbox{\hrule width 3pt depth -1.5pt height 1.9pt
      \vskip -1.5pt
      \hbox{\hskip 1.3pt\vrule height 3pt depth 0pt width .4pt}}}

 
\def\xz{{\sf X^{\rm z}}}
\def\bxz{{\cal B}(\state^\hbox{\rm\tiny z})}
\def\xzplus{{\sf X^{{\rm z}_{ \tinyplus}}}}
\def\xbxm{({\sf X},{\cal B}({\bf X}),{\bf m})}
\def\bx{{{\cal B}(\state)}}
\def\bxzplus{{\cal B}(\state^{{\rm z}_{\tinyplus}} )} \def\bxplus{{\clB^+(\state)}}


 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CHECKED CHARACTERS



\def\cclF{{\check{\clF}}}
\def\catom{{\check{\atom}}}
\def\cExpect{\check{\Expect}}
\def\cPhi{\check{\Phi}}
\def\cbfPhi{\check{\bfPhi}}
\def\cProb{\check{\Prob}}
\def\cProbsub{\cProb\!}
\def\cPhi{\check{\Phi}}

\def\cpi{\check{\pi}}
\def\cA{\check{A}}

\def\cG{{\check{G}}}

\def\cP{{\check{P}}}
\def\cbxplus{{\cal B}^+(\cstate)}
\def\cstate{{\check{\state}}}
\def\bcx{\clB(\cstate)}

\def\LPhi{\bfPhi^{\Lambda}} 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BF PREFIXES


\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfC{{\bf C}}
\def\bfD{{\bf D}}
\def\bfE{{\bf E}}
\def\bfF{{\bf F}}
\def\bfG{{\bf G}}
\def\bfH{{\bf H}}
\def\bfI{{\bf I}}
\def\bfJ{{\bf J}}
\def\bfK{{\bf K}}
\def\bfL{{\bf L}}
\def\bfM{{\bf M}}
\def\bfN{{\bf N}}
\def\bfO{{\bf O}}
\def\bfP{{\bf P}}
\def\bfQ{{\bf Q}}
\def\bfR{{\bf R}}
\def\bfS{{\bf S}}
\def\bfT{{\bf T}}
\def\bfU{{\bf U}}
\def\bfV{{\bf V}}
\def\bfW{{\bf W}}
\def\bfX{{\bf X}}
\def\bfY{{\bf Y}}
\def\bfZ{{\bf Z}}

\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfc{{\bf c}}
\def\bfd{{\bf d}}
\def\bfe{{\bf e}}
\def\bff{{\bf f}}
\def\bfg{{\bf g}}
\def\bfh{{\bf h}}
\def\bfi{{\bf i}}
\def\bfj{{\bf j}}
\def\bfk{{\bf k}}
\def\bfl{{\bf l}}
\def\bfm{{\bf m}}
\def\bfn{{\bf n}}
\def\bfo{{\bf o}}
\def\bfp{{\bf p}}
\def\bfq{{\bf q}}
\def\bfr{{\bf r}}
\def\bfs{{\bf s}}
\def\bft{{\bf t}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfw{{\bf w}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfz{{\bf z}}




%bfsymbols


\def\bfmath#1{{\mathchoice{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$\scriptstyle#1$}}%
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}
 
 
\def\bfPhi{\bfmath{\Phi}}
\def\bfPsi{\bfmath{\Psi}}
\def\bfGamma{\bfmath{\Gamma}}
\def\bfDelta{\bfmath{\Delta}}

\def\bfTheta{\bfmath{\Theta}}

\def\bfiota{\bfmath{\iota}}
\def\bflambda{\bfmath{\lambda}}
 \def\bfphi{\bfmath{\phi}}



\def\bfxi{\bfmath{\xi}}
 \def\bfzeta{\bfmath{\zeta}}
\def\bftheta{\bfmath{\theta}}
\def\bftiltheta{\bfmath{\tiltheta}}
\def\bfhatheta{\bfmath{\hatheta}}
\def\bfvarphi{\bfmath{\varphi}}
\def\bfpsi{\bfmath{\psi}}
\def \bfpi {\bfmath{\pi}}
\def\bfeta{\bfmath{\eta}} 
 
 
%boldmath

%%%


\def\bfma{\bfmath{a}}
\def\bfmb{\bfmath{b}}
\def\bfmd{\bfmath{d}}
\def\bfme{\bfmath{e}}
\def\bfmm{\bfmath{m}}
\def\bfmq{\bfmath{q}}
\def\bfmr{\bfmath{r}}

\def\bfmmu{\bfmath{\mu}}   
\def\bfnu{\bfmath{\nu}}   
%\def\bfgamma{\bfmath{\gamma}}   


\def\bfmu{\bfmath{u}} 
\def\bfmv{\bfmath{v}} 
\def\bfmx{\bfmath{x}}
\def\bfmy{\bfmath{y}}
\def\bfmw{\bfmath{w}}
 

\def\bfmhaw{\bfmath{\haw}}  

\def\bfmz{\bfmath{z}}  

\def\bfmA{\bfmath{A}}
\def\bfmB{\bfmath{B}}  

\def\bfmC{\bfmath{C}} 
\def\bfmD{\bfmath{D}} 
\def\bfmE{\bfmath{E}}   
\def\bfmF{\bfmath{F}}     
\def\bfmG{\bfmath{G}}     
\def\bfmH{\bfmath{H}}     
\def\bfmI{\bfmath{I}}      
\def\bfmhaI{\bfmath{\haI}}   
\def\bfmhaL{\bfmath{\haL}}     
\def\bfmL{\bfmath{L}}
\def\bfmM{\bfmath{M}}
\def\bfmN{\bfmath{N}}  
\def\bfmQ{\bfmath{Q}}  
\def\bfmR{\bfmath{R}}  
\def\bfmbarR{\bfmath{\bar{R}}}  
 

 
 

\def\bfmS{\bfmath{S}}  
\def\bfmT{\bfmath{T}}  
\def\bfmU{\bfmath{U}}  
 

\def\bfmhaN{\bfmath{\widehat N}}
\def\bfmhaQ{\bfmath{\widehat Q}}
 
\def\bfmX{\bfmath{X}}
\def\bfmtilX{\bfmath{\widetilde{X}}}

\def\bfmtilQ{\bfmath{\widetilde{Q}}}

\def\bfmtilq{\tilde{\bfmath{q}}}


%\def\bfmtilX{\tilde \bfmX}


\def\bfmY{\bfmath{Y}}   
\def\bfmhaY{\bfmath{\widehat Y}}


\def\bfmhhaY{\bfmath{\hhaY}} %\widehat{\widehat{Y}}}}
\def\bfmhhaY{\hbox to 0pt{$\widehat{\bfmY}$\hss}\widehat{\phantom{\raise 1.25pt\hbox{$\bfmY$}}}}
 

\def\bfmW{\bfmath{W}}  
\def\bfmhaW{\bfmath{\haW}}  
\def\bfmZ{\bfmath{Z}}  



\def\bfmhaq{\bfmath{\widehat q}}
\def\bfmhaw{\bfmath{\widehat w}}
\def\bfmhay{\bfmath{\widehat y}}
\def\bfmhaz{\bfmath{\widehat z}}
\def\bfmhaQ{\bfmath{\widehat Q}}
\def\bfmhaS{\bfmath{\widehat S}}
\def\bfmhaU{\bfmath{\widehat U}}
\def\bfmhaW{\bfmath{\widehat W}}









% \ha prefixes

%  Hat

\def\haPsi{{\widehat{\Psi}}}
\def\haGamma{{\widehat{\Gamma}}}
\def\haSigma{{\widehat{\Sigma}}}
\def\habfPhi{{\widehat{\bfPhi}}}

\def\haPi{{\widehat \Pi}}


\def\haP{{\widehat P}}
\def\haZ{{\widehat Z}}




\def\haf{{\hat f}}
\def\hag{{\hat g}}
\def\hah{{\hat h}}
\def\ham{{\hat m}}
\def\hay{{\widehat y}}
\def\hav{\hat v}
\def\hatheta{{\hat\theta}}
\def\hapsi{{\hat\psi}}
\def\hanu{{\hat\nu}}
\def\hamu{{\hat\mu}}
\def\halpha{{\hat\alpha}}
\def\habeta{{\hat\beta}}
\def\hagamma{{\hat\gamma}}

\def\haphi{\hat{\phi}}


\def\hanabla{\widehat{\nabla}}


\def\halambda{{\hat\lambda}}
\def\haLambda{{\hat\Lambda}}


\def\haA{\widehat A}
\def\haK{\widehat K}


\def\haT{\widehat T}
\def\haX{\widehat X}

% \rm prefixes



\def\rmA{{\rm A}}
\def\rmB{{\rm B}}
\def\rmC{{\rm C}}
\def\rmD{{\rm C}}
\def\rmE{{\rm E}}
\def\rmH{{\rm H}}
\def\rmI{{\rm I}}
\def\rmM{{\rm M}}
\def\rmP{{\rm P}}
\def\rmQ{{\rm Q}}
\def\rmT{{\rm T}}

\def\rmd{{\rm d}}
\def\rmg{{\rm g}}
\def\rmk{{\rm k}}
\def\rms{{\rm s}}
\def\rmu{{\rm u}}
\def\rmx{{\rm x}}

\def\rmP{{\rm P}}
\def\rmE{{\rm E}}


 

% Wide tilde


 
\def\tilDelta{{\widetilde \Delta}}
\def\tilGamma{{\widetilde \Gamma}}
\def\tilPhi{{\widetilde \Phi}}
\def\tilL{{\widetilde L}}


\def\tilA{\tilde{A}}

\def\tilM{{\widetilde M}}
\def\tilN{{\widetilde N}}
\def\tilP{{\widetilde P}}
\def\tilQ{{\widetilde Q}}
\def\tilR{\widetilde R}

\def\tilbfmQ{\bfmath{\widetilde Q}}


\def\tilT{\widetilde T}
\def\tilU{\widetilde U} 
\def\tilV{\widetilde V} 
\def\tilW{\widetilde W}
\def\tilX{\widetilde X}
\def\tilY{\widetilde Y}


\def\tilbfX{{\bf\widetilde X}}


\def\tilbfmM{\bfmath{\widetilde M}}  
\def\tilbfmN{\bfmath{\widetilde N}}  
\def\tilbfmQ{\bfmath{\widetilde Q}} 
 
% Tilde


\def\tilb{{\tilde b}}

\def\tilphi{{\tilde \phi}}


\def\tilmu{{\tilde \mu}}
\def\tilnu{{\tilde \nu}}
\def\tilpi{{\tilde \pi}}
\def\tilsigma{\tilde \sigma}
\def\tiltau{\tilde \tau}

\def\tiltheta{{\tilde \theta}}

\def\tilpsi{{\widetilde \psi}}

\def\tilc{\tilde c}
\def\tile{\tilde e}
\def\tilf{\tilde f}
\def\tilg{\tilde g}
\def\tilr{\tilde r}
\def\tilv{\tilde v}
\def\tilx{\tilde x}
\def\tily{\tilde y}


\def\tilbfm{{\bf \tilde  m}}





%Caligraphy

%%%  careful, used for too many things:  \def\clA{{\cal A}}
\def\clB{{\cal B}}
\def\clC{{\cal C}}
%%%  careful, used for too many things:  \def\clD{{\cal D}}
\def\clE{{\cal E}}
\def\clF{{\cal F}}
\def\clG{{\cal G}}
\def\clH{{\cal H}}
\def\clJ{{\cal J}}
\def\clI{{\cal I}}
\def\clK{{\cal K}}
\def\clL{{\cal L}}
\def\clM{{\cal M}}
\def\clN{{\cal N}}
\def\clO{{\cal O}}
\def\clP{{\cal P}}
\def\clQ{{\cal Q}}
\def\clR{{\cal R}}
\def\clS{{\cal S}}
%\def\clT{{\cal T}}
\def\clU{{\cal U}}
\def\clV{{\cal V}}
\def\clW{{\cal W}}
\def\clX{{\cal X}}
\def\clY{{\cal Y}}
\def\clZ{{\cal Z}}

  
 
\def\clL{{\cal L}}
\def\clI{{\cal I}}
\def\clC{{\cal C}}

\def\tilclE{\tilde{\clE}}
\def\tilbfmclE{\bfmath{\tilde{\clE}}}

\def\tilq{\tilde{q}}
\def\tilbfmq{\bfmath{\tilde{q}}}

\def\bfmclQ{\bfmath{\clQ}}   

\def\bfmclE{\bfmath{\clE}}  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISCELLANEOUS

\def\bcbm{b_{\hbox{{\rm\tiny CBM}}}}
 
\def\Gexp{\clG^+(\gamma)}
\def\Gexps{\clG^+(s)}

 

%\def\sfhead#1{\subsection*{\sf#1}}
 

\def\implies{\Rightarrow}
  

 
\def\eqdef{\mathbin{:=}}

\def\lebmeas{\mu^{\hbox{\rm \tiny Leb}}}
\def\Prbty{{\cal  M}}
\def\Prob{{\sf P}}
\def\Probsub{{\sf P\! }}
\def\Expect{{\sf E}}

\def\Var{\hbox{\sf Var}}
\def\Cov{\hbox{\sf Cov}}
\def\CV{\hbox{\sf CV}}


\def\lgmath#1{{\mathchoice{\mbox{\large #1}}%
{\mbox{\large #1}}%
{\mbox{\tiny #1}}%
{\mbox{\tiny #1}}}}


\def\One{{\mathchoice{\lgmath{\sf 1}}%
{\mbox{\sf 1}}%
{\mbox{\tiny \sf 1}}%
{\mbox{\tiny \sf 1}}}}

\def\Zero{{\mathchoice{\mbox{\sf 0}}%  \lgmath
{\mbox{\sf 0}}%
{\mbox{\tiny \sf 0}}%
{\mbox{\tiny \sf 0}}}}



\def\taboo#1{{{}_{#1}P}}

\def\tinybull{\hbox{\tiny$\ddag$}}

\def\bullP{{{}_{\tinybull}P}}

\def\bullX{X_{\tinybull}}
\def\bfmbullX{\bfmX_{\tinybull}}
\def\bullstate{\state_{\tinybull}}
\def\bullx{x^{\tinybull}}
\def\bullh{h_{\tinybull}}
\def\bullc{c_{\tinybull}}
\def\bulltau{\tau_{\tinybull}}


%\def\bullX{{{}_{\tinybull}X}}
%\def\bfmbullX{{{}_{\tinybull}\bfmX}}
%\def\bullstate{{{}_{\tinybull}\state}}
 


\def\io{{\rm i.o.}}
    

\def\as{{\rm a.s.}}
\def\Vec{{\rm vec\, }}

 \def\Tol{\text{\rm Tol}}




\def\ind{\bbbone}
  
 \def\epsy{\varepsilon}

\def\varble{\,\cdot\,}




\def\formtmp#1#2{{\vskip12pt\noindent\fboxsep=0pt\colorbox{#1}{\vbox{\vskip3pt\hbox to \textwidth{\hskip3pt\vbox{\raggedright\noindent\textbf{#2\vphantom{Qy}}}\hfill}\vspace*{3pt}}}\par\vskip2pt%
\noindent\kern0pt}}

 
 
                        

 
%  Warning:  \endlinechar fixes line skip at start, but may create other issues.  The value 13 is default.
\newenvironment{programcode}[1]{\ignorespaces\def\stmtopen##1{##1}%
\pagebreak[3]%
\formtmp{programcode}{#1}%
%\ignorespacesafterend%
\endlinechar=-1\relax%
%\catcode\endlinechar=9\relax%
\nopagebreak[4]}{%
\noindent\textcolor{programcode}{\rule{\columnwidth}{1pt}}\vskip1pt\par\addvspace{\baselineskip}%
\endlinechar=13}
 
     %%%%   NOTE:   (for IEEE)
     



\renewenvironment{programcode}[1]{\smallbreak\noindent\textbf{#1}\quad \gobblepars}{}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  underbar prefixes  

 
\def\uT{\hbox{\underbar{$T$}}}
\def\uI{\underbar{$I$}}
\def\uN{\underbar{$N$}}

\def\unc{{\hbox{\underbar{$c$}}}}

 
\def\undern{{\underline{n}}}
\def\ubarho{{\underline{\rho}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
  
 
\def\bara{{\overline {a}}}
\def\barb{{\overline {b}}}
\def\barc{{\overline {c}}}


   \def\ubarc{\underline{c}}
   \def\ubarw{\underline{w}}
   \def\ubary{\underline{y}}
   
    
\def\bare{\bar{e}}
\def\barclE{\bar{\clE}}
\def\barcx{{\barc}_{\hbox{\it\tiny X}}}

\def\barcy{{\barc}_{\hbox{\it\tiny Y}}}

\def\bard{{\overline {d}}}

\def\barf{{\overline {f}}}
\def\barg{{\overline {g}}}
\def\barh{{\overline {h}}}
\def\bark{{\overline {k}}}
\def\barI{{\overline {l}}}
\def\barm{{\overline {m}}}
\def\barn{{\overline {n}}}

\def\barp{{\overline {p}}}
\def\barq{{\overline {q}}}
\def\barr{{\overline {r}}}
\def\bars{{\overline {s}}}
\def\barv{{\overline {v}}}
\def\barw{{\overline {w}}}
\def\barx{{\overline {x}}}
\def\bary{{\overline {y}}}
 
 
\def\barA{{\bar{A}}}
\def\barB{{\bar{B}}}
\def\barC{{\bar{C}}}
\def\barD{{\bar{D}}}
\def\barE{{\bar{E}}}
\def\barH{{\bar{H}}}
\def\barJ{{\bar{J}}}
\def\barL{{\bar{L}}}
\def\barP{{\bar{P}}}
\def\barQ{{\bar{Q}}}
\def\barR{{\bar{R}}}
\def\barS{{\bar{S}}}
\def\barT{{\bar{T}}}
\def\barU{{\bar{U}}}
\def\barX{{\bar{X}}}
\def\barY{{\bar{Y}}}
\def\barZ{{\bar{Z}}}
 
 

\def \barzeta{{\overline{\zeta}}}

\def\baratom{{\overline{\atom}}}

\def\bareta{{\overline{\eta}}}
\def\barho{{\overline{\rho}}}
\def\barmu{{\overline{\mu}}}
\def\barnu{{\overline{\nu}}}

\def\bartheta{{\overline{\theta}}}

\def\barTheta{{\overline{\Theta}}}

\def\barpsi{{\bar{\psi}}}


\def\barnabla{\bar{\nabla}}

\def\barlambda{\bar \lambda}


\def\baralpha{{\bar{\alpha}}}
\def\barbeta{{\bar{\beta}}}

\def\barepsy{{\bar{\epsy}}}
\def\barvarpi{{\bar{\varpi}}}

\def\barbP{\overline{\bfPhi}}
\def\barPhi{\overline{\Phi}}
\def\barF{\overline{\clF}}
\def\barsigma{\overline{\sigma}}

\def\barSigma{\overline{\Sigma}}
\def\barDelta{\overline{\Delta}}
\def\barGamma{\overline{\Gamma}}
\def\barLambda{\overline{\Lambda}}


\def\bartau{\overline{\tau}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASSUMPTIONS

               

\newenvironment{assumptions}[1]{% 
\setcounter{keep_counter}{\value{#1}}
\def\aref{#1}
\begin{list}{\sf\, (#1\arabic{#1})\mindex{Assumption (#1\arabic{#1})}\, }{\usecounter{#1}%
\setlength{\rightmargin}{\leftmargin}}
\setcounter{#1}{\value{keep_counter}}}%
{\end{list}}



\def\ass(#1:#2){(#1\ref{#1:#2})}
 

\def\ritem#1{
\item[{\sf \ass(\current_model:#1)}]
}

\newenvironment{recall-ass}[1]{% 
\begin{description}
\def\current_model{#1}}{
\end{description}
} 

 


\def\MT{\cite{meytwe92d}}
  
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% qed
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\sq\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\sq
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

%\renewenvironment{proof}{\vspace{1ex}\noindent{\bf Proof}\hspace{0.5em}}%
%{\hfill\qed\vspace{1ex}}
 
\newcommand{\blot}{\vrule height 1.1ex width .9ex depth -.1ex }
\def\qedb{\ifmmode\blot\else{\vspace{-.2cm}\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\blot
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}



 

  



  


%        \renewenvironment{thebibliography}[1]
%          {\section*{\centering\normalfont\small\MakeUppercase{#1}}\small
%           \begin{list}{}{\setlength{\leftmargin}{\bibindent}
%                          \setlength{\itemindent}{-\leftmargin}
%                          \setlength{\itemsep}{0pt}
%                          \setlength{\parsep}{\smallskipamount}
%                          \usecounter{enumiv}\renewcommand{\theenumiv}{}}
%           \sloppy\clubpenalty=4000\widowpenalty=4000\frenchspacing}
%          {\end{list}}  
     
\newcounter{rmnum}
\newenvironment{romannum}{\begin{list}{{\upshape (\roman{rmnum})}}{\usecounter{rmnum}
\setlength{\leftmargin}{8pt}
\setlength{\rightmargin}{6pt}
\setlength{\itemindent}{0pt}
}}{\end{list}}

\newcounter{anum}
\newenvironment{alphanum}{\begin{list}{{\upshape (\alph{anum})}}{\usecounter{anum}
\setlength{\leftmargin}{8pt}
\setlength{\rightmargin}{6pt}
\setlength{\itemindent}{0pt}
}}{\end{list}}
  



%
%%\newenvironment{exercises}{%  
%%\clearpage
%%\section{Exercises} 
%%\begin{list} 
%%%\setcounter{exercise}{0}
%%{\textbf{\thechapter.\textit{\arabic{exercise}}}}{\usecounter{exercise}}%
%%\setlength{\topsep}{0pt}
%%\setlength{\partopsep}{0pt}
%%\setlength{\itemsep}{0pt}
%%\setlength{\parsep}{5pt}
%%\setlength{\leftmargin}{-10pt}
%%\setlength{\rightmargin}{0pt}
%%\setlength{\itemindent}{-5pt} 
%%}
%%{\end{list}
%%\bigbreak}


%\newcounter{exercise}

%\newlist{EX}{enumerate}{1}
%\setlist[EX]{label=\thechapter.\arabic*,%
%topsep=0pt,%
%partopsep=0pt,%
%listparindent = 0pt,%
%itemsep=0pt,%
%parsep=3pt,%
%labelwidth=15pt,%
%labelsep=10pt,%
%leftmargin=25pt,% 
%itemindent=-5pt,%
%rightmargin=0pt,%
%itemindent=0pt,%
%}


%\newenvironment{exercises}{
%\clearpage
%\section{Exercises}   
%\begin{EX}}{\end{EX}}
% 
  
 
\def\vecrho{\vec{\rho}}
 
\newcommand{\field}[1]{\mathbb{#1}} 

\def\posRe{\field{R}_+}
\def\Re{\field{R}} 

\def\intgr{\field{Z}}
\def\nat{\field{Z}_+}

\def\A{\field{A}}     
  
  \def\rat{\field{Q}}

\def\Co{\field{C}}

\def\Prob{{\sf P}}
\def\Probsub{{\sf P\! }}
\def\Expect{{\sf E}}


\def\Z{{\sf Z}}




 
\def\hasC{\widehat{\sf C}}

\def\B{{\sf B}} 

 

 
% Special symbols

\def\transpose{{\intercal}}

% \def\transpose{{\hbox{\rm\tiny T}}}

\def\rank{{\rm rank\,}}
\def\closure{{\rm closure\,}}
\def\interior{{\rm interior\,}}

\def\deg{\hbox{\rm deg\thinspace}}
\def\diag{\hbox{\rm diag\thinspace}}

 
\def\Real{\text{\rm Re\,}}

\def\st{\text{\rm s.t.\,}}

\def\sign{{\rm sign}}
\def\supp{{\rm supp\,}}
\def\argmin{\mathop{\rm arg\, min}}
\def\ind{\hbox{\large \bf 1}}

 
%\def\atom{{\mathchoice{\bftheta}{\bftheta}{\theta}{\theta}}}    MANY defs!
\def\atom{{x^\bullet}}

\def\aatom{{x^{\bullet\bullet}}}

\def\trace{\hbox{\rm trace\,}}  
\def\epsy{\varepsilon}
\def\varble{\,\cdot\,} 
\def\dint{\mathop{\int\!\!\!\int}} 

%%\def\stationA{\hbox{\small$\mathcal S$}}
%%\def\stationB{\hbox{\tiny$\mathcal S$}}
%%\def\station{{\mathchoice{\stationA}{\stationA}{\stationB}{\stationB}}}  
%
%%\def\stationA{\hbox{s}}
%%\def\stationB{\hbox{\small s}}
%%\def\station{{\mathchoice{\stationA}{\stationA}{\stationB}{\stationB}}}  
% 
%
%%\def\resourceA{\hbox{\small$\mathcal S$}}
%%\def\resourceB{\hbox{\tiny$\mathcal S$}}
%%\def\resource{{\mathchoice{\resourceA}{\resourceA}{\resourceB}{\resourceB}}}  

%
%%\def\resourceA{\hbox{r}}
%%\def\resourceB{\hbox{\small r}}
%%\def\resource{{\mathchoice{\resourceA}{\resourceA}{\resourceB}{\resourceB}}}  


\def\station{s}
\def\resource{r}

 \def\clIp{\clI^{\hbox{\tiny$\mathcal P$}}} 
 
 
  
% Tilde symbols


\def\wtilde{\widetilde{\normalsize\rule{0cm}{1.3ex}\bfw\rule{0cm}{1.4ex}}}
\def\tilw{\widetilde{w}}
\def\tillambda{\widetilde{\lambda}}


% Hat symbols

 
 
\def\zetass{\zeta^{\hbox{\tiny e}}}

\def\hazeta{\widehat\zeta}


\def\haH{\widehat{H}}

\def\haJ{\widehat J}  
\def\haL{\widehat L}  
\def\haN{\widehat{N}}
\def\haV{\widehat{V}}
\def\haW{\widehat{W}}
\def\haY{\widehat{Y}}


%\def\hhaY{\widehat{\widehat{Y}}}
 
\def\hhaY{\hbox to 0pt{$\haY$\hss}\widehat{\phantom{\raise 1.25pt\hbox{Y}}}}
 
\def\haXi{\widehat{\Xi}}

\def\haXiy{{\widehat{\Xi}_{\scriptscriptstyle Y }}}

\def\Xiy{\Xi_{\scriptscriptstyle Y}}
 

\def\hab{\widehat b}
\def\haq{\widehat q}
\def\haw{\widehat w}
\def\hax{\widehat x}
\def\haz{\widehat z}


\def\haA{\widehat A}

\def\haC{{\widehat C}}
\def\haG{{\widehat G}}
\def\haI{{\hat I}}
\def\haM{{\widehat M}}
\def\haQ{{\widehat Q}}
\def\haS{{\widehat S}}
\def\haU{{\widehat U}}
\def\haY{\widehat Y} 

\def\haeta{\widehat\eta}
 

% 


\def\hasU{\widehat{\sf U}}
\def\hasV{\widehat{\sf V}}
\def\hasW{\widehat{\sf W}}
\def\hasY{\widehat{\sf Y}}


 
% Bold symbols



\def\bfmf{\bfmath{f}}   
\def\bfmF{\bfmath{F}}   


\def\bfclE{\bfmath{\clE}}
\def\bfclG{\bfmath{\clG}}
\def\bfclW{\bfmath{\clW}}
\def\bfclZ{\bfmath{\clZ}}

%\def\pp{\bfmath{p$}}}
   

 


\def\bfatom{\bfmath{\theta}}
\def\bfPhi{\bfmath{\Phi}}
\def\bfpi{\bfmath{\pi}} 
\def\bfrho{\bfmath{\rho}}
\def\bfUpsilon{\bfmath{\Upsilon}} 



 

  
  
  
  
  
  
   
      

\newcommand{\inD}{\mbox{ $\Rightarrow$ }}

  

\def\down{{\hbox{\tiny down}}}

\def\tinyD{{\hbox{\tiny D}}}




\def\discountMark{{\hbox{\small$\star$}}}
 

\def\OPT{(\ref{e:OE1},\ref{e:OE2})}
     
     

\def\generate{{\cal A}}  % no D

 
\def\tinyCLT{{\hbox{\rm\tiny CLT}}} 
\def\sigmaCLT{\sigma_\tinyCLT}
\def\hasigmaCLT{\widehat{\sigma}_\tinyCLT}

\def\barsigmaCLT{\barsigma_\tinyCLT}

%%  Little rover


\def\Top{{\tt T}}
\def\Roll{{\tt R}}
\def\Bot{{\tt B}}


\def\Dri{{\tt D}}
\def\DD{ \cancel{\tt D}}

 

  
 %%%%%%%%%%%%%%%%%%%%%%%%%%%% FOR SAMPLED CHAINS IN CH{CRITERIA}

\def\Sampsigma{\hat{\sigma}}
\def\Samptau{\hat{\tau}}
\def\SampP{\widehat{P}}
\def\SampX{\widehat{X}}
\def\SampbfX{\widehat{\bfmX}}
\def\SampF{\widehat{\cal F}}




